Federated Learning for Inference at Anytime and Anywhere

Federated learning has been predominantly concerned with collaborative training of deep networks from scratch, and especially the many challenges that arise, such as communication cost, robustness to heterogeneous data, and support for diverse device capabilities. However, there is no unified framework that addresses all these problems together. This paper studies the challenges and opportunities of exploiting pre-trained Transformer models in FL. In particular, we propose to efficiently adapt such pre-trained models by injecting a novel attention-based adapter module at each transformer block that both modulates the forward pass and makes an early prediction. Training only the lightweight adapter by FL leads to fast and communication-efficient learning even in the presence of heterogeneous data and devices. Extensive experiments on standard FL benchmarks, including CIFAR-100, FEMNIST and SpeechCommandsv2 demonstrate that this simple framework provides fast and accurate FL while supporting heterogenous device capabilities, efficient personalization, and scalable-cost anytime inference.

==> old_method_accumulator.tex <==
\subsection{\alg{}}
\label{sec:accumulator}
%To adapt a pre-trained Transformer model, namely its encoder, into a downstream task, 
We inject our Accumulator into each of the self-attention blocks followed by a shared MLP head to enable early predictions. 
%. We will only detail our Accumulator here as MLP head is widely known nowadays. 
%Specifically, our Accumulator modulates the [CLS] token embedding produced from any layer of a pretrained Transformer and enables a shortcut between each Transformer layer and the final MLP head for predictions.
% propose a novel adapter \steve{adapter and accumulator are getting mixed together as terms} termed \emph{\alg{}} to conduct the parameter-efficient learning. 

\paragraph{Feature Modulation.} Given the feature embedding from any block of a pretrained Transformer, it will be modulated by our \alg{}.
Our \alg{} is a single-block Transformer encoder, which can input a sequence of the [CLS] tokens output from up to any layer of a pre-trained Transformer. Therefore the input for our \alg{} becomes 
\begin{equation}
\begin{aligned}
    \mathbf{h}_{\text{in}, l} &= [\mathrm{h}_{\text{cls}}; \mathbf{z}_1^0; \cdots;\mathbf{z}_l^0] + \mathbf{p}'_{[1:l]} = A \circ S^l_{\theta} \circ T(\mathbf{x}), \quad l \in [1, L],
    \label{eq:ourz0}
\end{aligned}
\end{equation}
where $\mathrm{h}_{\text{cls}}$ and $\mathbf{p}'$ are the learnable [CLS] token and positional embedding randomly initialized in our \alg{}. $\mathbf{z}_l^0 = S^l_\theta(\mathbf{z}_0)^0$
% \footnote{TODO:Need to add the CLS token exchanging.} 
is the [CLS] token embedding output from layer $l$ of a pre-trained Transformer. Note that now the positional information embedded in $\mathbf{p}'$ corresponds to different layers in the pre-trained Transformer. $A(.)$ is a special tokenization function that accumulates the [CLS] token of \alg{} and the [CLS] tokens output from $S^1_{\theta}$ to $S^l_{\theta}$ of the pre-trained Transformer for input $\mathbf{x}$ and converts them into a sequence input.

Now our \alg{} can be briefly formalized as
\begin{equation}
\begin{aligned}
    \mathbf{h}_{\text{out}, l} = S^1_{\psi} \circ A \circ S^l_{\theta} \circ T(\mathbf{x}), 
    % \text{where} ~~~ F_{\theta} (\mathbf{z}_0) &= F^L_{\theta}\circ\cdots\circ F^1_{\theta} (\mathbf{z}_0), \\
    % F^l_{\theta} (\mathbf{z}_0) &= \text{MLP}^*(\text{LN}(\text{MSA}^*(\text{LN}(\mathbf{z}_{l-1}))
\end{aligned}
\end{equation}
where $\psi$ is the parameters of our \alg{} as a one block Transformer encoder $S^1_{\psi}$\footnote{We abuse the function notation $S()$ defined above to represent the self-attention block of our \alg{} for simplicity.}. $\mathbf{h}_{\text{out},l}^0$ then will be fed into an MLP head to predict labels. Note that $\mathbf{z}_l^0$ will be replaced by the transformed token $\mathbf{h}_{\text{out},l}^0$ during the feature propagation when $l<L$. And when computing $\mathbf{h}_{\text{out}, l}$ residual connection is applied over $\mathbf{z}_l^0$ from $S^l_{\theta} \circ T(\mathbf{x})$.

\paragraph{Early Predictions.} One nice property of our framework is we can make early predictions for the modulated feature from any block of a pre-trained Transformer. Once we get the modulated feature $\mathbf{h}_{\text{out},l}^0$ from block $l$, it can be fed into the MLP head to get the prediction
$$\hat{y}^l = G_{\phi}(\mathbf{h}_{\text{out},l}^0) = G_{\phi}\circ S^1_{\psi} \circ A \circ S^l_{\theta} \circ T(\mathbf{x}).$$
% $\hat{y}^l$ is the prediction from layer $l$ of $S_{\theta}$.

While, at the training stage, the model can be optimized as 
\begin{equation}\label{eq:peofacm}
\begin{aligned}
    \phi, \psi &= \underset{\phi, \psi}{\arg\min}  \frac{1}{M}\sum_{j=1}^{M}\ell(\hat{y}_j^l, y_j)  = \underset{\phi, \psi}{\arg\min}  \frac{1}{M}\sum_{j=1}^{M}\ell(G_{\phi}\circ S^1_{\psi} \circ A \circ S^l_{\theta} \circ T(\mathbf{x}_j), y_j ),
\end{aligned}
\end{equation}
where the parameters $\phi, \psi$ are the only trainable parameters during training. Different devices can make early predictions using different sets of layers $l$, which will be important for supporting device heterogeneity.
%And $l$ can be set differently in the optimization for different devices, which is important for FL as stated next. 
% Specifically, larger $l$ may correspond to devices with larger compute capabilities. Thus, our FL system can be trained among clients with heterogeneous computing capabilities.

% \steve{Define somewhere the added residual connection in the accumulator that accelerates convergence.}


\subsection{Federated \alg{}}
Our goal is to adapt a pre-trained Transformer FM via federated learning of our \alg{}. As stated in Section~\ref{sec:fl}, in FL, there are typically $K$ different clients, which may or may not have the same computational constraints. 

\paragraph{Learning.}
Now the learning objective of Eq.~\ref{eq:global} becomes 
\begin{equation}\label{eq:flacm}
    \phi, \psi = \underset{\phi, \psi}{\arg\min} \sum_{i=1}^k \alpha_i \mathcal{L}_i(\phi, \psi), \quad \mathcal{L}_i(\phi, \psi)= \frac{1}{N_i}\sum_{j=1}^{N_i}\ell(\hat{y}^l_j, y_j),
\end{equation}
where $k$ is the number of sampled clients for FL training each round with typically $k<<K$, $S^{L_i}_{\theta}$ means the blocks can be used for the feed-forward pass for client $i$ until block $L_i$. Our \alg{} and MLP head are the only modules learned during FL. Note that $L_i\in[1, L]$ can be decided by the computational constraint in each client $i$, i.e. a client with more compute power can have a larger $L_i$. This attribute is important to FL as now our framework can conduct the federated learning flexibly among clients with different compute capabilities.

\paragraph{Personalization.} Interestingly,  our \alg{} $G_\phi \circ S^1_{\psi}$ can be rapidly personalized following Eq.~\ref{eq:per} on a local device after the FL training. Because it is parameter light, this is both computationally efficient and feasible to perform on limited local client data, in contrast to full network fine-tuning, which could easily overfit in a limited data regime.

\paragraph{Inference.} Given an FL trained model in client $i$, it can not only infer labels $\hat{y}^{L_i}$ from block $L_i$ according to its capability but also it can infer labels $\hat{y}^{l_i}$ as long as $l_i$ is smaller than the layer constraint $L_i$. This property is very useful. For example, when the user device, such as a cellphone, is used with a (low) battery, they can set small $l_i<L_i$ for fast inference to save battery cost. 

==> tabs/ablation.tex <==
\begin{table}[t]
    \vspace{-2em}
    \caption{Ablation study on Accumulator.}
    \centering
    \scalebox{1.0}{
    \begin{tabular}{l|c}
    \toprule
    \multirow{1}{*}{}\Tstrut & Mean performance\\
    \midrule
    Full Accumulator &  \multirow{}{*}{64.28}\\
    \midrule
    Depth=3 & 64.55 (+0.25)\\
    \midrule
    No Replace & 64.74 (-2.59) \\
    \midrule
    No Residual & 59.80 (-4.48)\\
    \midrule
    No Adapter & 64.01 (-0.54)\\
    \midrule
    Linear Head &  62.36 (-2.19)\\
    \bottomrule
    \end{tabular}
}
    \label{tab:ablation}
\end{table}

==> tabs/exp4.tex <==
\begin{table}[t]
\caption{Personalized performance on CIFAR-100 with multi-tier constraints after FL training on CIFAR-100.}
\centering
\scalebox{1.0}{
\begin{tabular}{l|ccc|c}
\toprule
Update part for\Tstrut & \multicolumn{3}{c}{LDA Partition (Dirichlet $\alpha$)} & \multirow{2}{*}{Parameter Size} \\ 
\cmidrule{2-4}
  personalization & IID ($1000.0$) & Non-IID ($1.0$) & Non-IID ($0.1$) &  \\ \midrule
Full Model & &  & & 30.62M \\
\midrule
L.W. Linear + Adapter &&  & & 1.06M \\
Adapter Only &&  & & 0.60M \\
\midrule
L.W. MLP + Adapter &&  & & 9.55M \\
Adapter Only & &  & & 0.60M \\
\midrule
\alg{} + Adapter & &  & & 3.77M \\
Adapter Only & &  && 0.60M \\
Client Token Only & &  & & 0.384K \\
\bottomrule
\end{tabular}
}
\label{tab:exp4}
\end{table}
